Brownian Paths Homogeneously Distributed in Space: Percolation Phase Transition and Uniqueness of the Unbounded Cluster

We consider a continuum percolation model on $\R^d$, $d\geq 1$.For $t,\lambda\in (0,\infty)$ and $d\in\{1,2,3\}$, the occupied set is given by the union of independent Brownian paths running up to time $t$ whoseinitial points form a Poisson point process with intensity $\lambda\textgreater{}0$.When $d\geq 4$, the Brownian paths are replaced by Wiener sausageswith radius $r\textgreater{}0$.We establish that, for $d=1$ and all choices of $t$, no percolation occurs,whereas for $d\geq 2$, there is a non-trivial percolation transitionin $t$, provided $\lambda$ and $r$ are chosen properly.The last statement means that $\lambda$ has to be chosen to be strictly smaller than the critical percolation parameter for the occupied set at time zero(which is infinite when $d\in\{2,3\}$, but finite and dependent on $r$ when $d\geq 4$).We further show that for all $d\geq 2$, the unbounded cluster in the supercritical phase is unique.Along the way a finite box criterion for non-percolation in the Boolean model is extended to radius distributions with an exponential tail. This may be of independent interest.The present paper settles the basic properties of the model and should be viewed as a jumpboard for finer results.

==> Bibfile.tex <==
\begin{thebibliography}{MMS86}

\bibitem[BK89]{BK89}
R.~M. Burton and M.~Keane.
\newblock Density and uniqueness in percolation.
\newblock {\em Comm. Math. Phys.}, 121(3):501--505, 1989.



\bibitem[GKN92]{GKN92}
A.~Gandolfi, M.~S. Keane, and C.~M. Newman.
\newblock Uniqueness of the infinite component in a random graph with
  applications to percolation and spin glasses.
\newblock {\em Probab. Theory Related Fields}, 92(4):511--527, 1992.

\bibitem[G61]{G61}
E.~N.~Gilbert.
\newblock Random Plane Networks.
\newblock{\em Journal of the Society for Industrial and Applied Mathematics,}
9(4): 533--543, 1961.



\bibitem[Gou08]{G08}
J.-B.~Gou{\'e}r{\'e}.
\newblock Subcritical regimes in the {P}oisson {B}oolean model of continuum
  percolation.
\newblock {\em Ann. Probab.}, 36(4):1209--1220, 2008.

\bibitem[Gri00]{G00}
G.~R.~Grimmett.
\newblock Percolation.
\newblock In {\em Development of mathematics 1950--2000}, pages 547--575.
  Birkh\"auser, Basel, 2000.

\bibitem[KS91]{KS91}
I.~Karatzas and S.~E.~Shreve.
\newblock {\em Brownian motion and stochastic calculus}, volume 113 of {\em
  Graduate Texts in Mathematics}.
\newblock Springer-Verlag, New York, second edition, 1991.

\bibitem[LSS97]{LSS97}
T.~M.~Liggett, R.~H.~Schonmann, and A.~M.~Stacey.
\newblock Domination by product measures.
\newblock {\em Ann. Probab.}, 25(1):71--95, 1997.

\bibitem[MMS88]{MMS88}
M.~V. Men{\cprime}shikov, S.~A. Molchanov, and A.~F. Sidorenko.
\newblock Percolation theory and some applications.
\newblock In {\em Probability theory. {M}athematical statistics. {T}heoretical
  cybernetics, {V}ol. 24 ({R}ussian)}, Itogi Nauki i Tekhniki, pages 53--110,
  i. Akad. Nauk SSSR Vsesoyuz. Inst. Nauchn. i Tekhn. Inform., Moscow, 1986.
\newblock Translated in J. Soviet Math. {{\bf{4}}2} (1988), no. 4, 1766--1810.

\bibitem[MP10]{MP10}
P.~M{\"o}rters and Y.~ Peres.
\newblock {\em Brownian motion}.
\newblock Cambridge Series in Statistical and Probabilistic Mathematics.
  Cambridge University Press, Cambridge, 2010.


\bibitem[MR94]{MR94}
R.~Meester and R.~Roy.
\newblock Uniqueness of unbounded occupied and vacant components in {B}oolean
  models.
\newblock {\em Ann. Appl. Probab.}, 4(3):933--951, 1994.

\bibitem[MR96]{MR96}
R.~Meester and R.~Roy.
\newblock {\em Continuum percolation}, volume 119 of {\em Cambridge Tracts in
  Mathematics}.
\newblock Cambridge University Press, Cambridge, 1996.

\bibitem[MRS94]{MRS94}
R.~Meester, R.~Roy, and A.~Sarkar.
\newblock Nonuniversality and continuity of the critical covered volume
  fraction in continuum percolation.
\newblock {\em J. Statist. Phys.}, 75(1-2):123--134, 1994.

\bibitem[Pen95]{P95}
M.~D.~Penrose.
\newblock Continuity of critical density in a boolean model.
\newblock {\em \emph{unpublished notes}}, 1995.

\bibitem[Szn10]{S10}
A.-S.~Sznitman.
\newblock Vacant set of random interlacements and percolation.
\newblock {\em Ann. of Math. (2)}, 171(3):2039--2087, 2010.

\end{thebibliography}
